Rethinking Shrinkage Bias in LLM FP4 Pretraining: Geometric Origin, Systemic Impact, and UFP4 Recipe

FP4 training promises substantial reductions in memory and computation cost for LLM pretraining, yet current FP4 hardware paths and recipes, including NVIDIA Blackwell/Rubin-class systems and AMD MI350-series GPUs, remain centered on E2M1 data elements. In this study, we identify a fundamental limitation of that choice: non-uniform formats such as E2M1 inherently suffer from Shrinkage Bias, a systematic negative rounding error caused by the geometric asymmetry of their representable bins. We show that this bias accumulates multiplicatively across layers and is amplified by the Random Hadamard Transform (RHT), providing a unified explanation for the training instability observed in existing E2M1-based FP4 recipes. In contrast, uniform grids (E1M2/INT4) bypass this grid-geometry error and better convert the improved bucket utilization from RHT into higher quantization quality. Based on this finding, we propose UFP4, a uniform 4-bit training recipe that applies RHT to all three training GEMMs while restricting stochastic rounding to dY alone. On Dense 1.5B, MoE 7.9B, and MoE 124B long-run pretraining, UFP4 consistently achieves lower BF16-relative loss degradation than strong E2M1-based baselines, supported by scaling-law analysis and ablation studies. Our results suggest that future accelerators should support E1M2/INT4-style uniform 4-bit grids as first-class training primitives alongside E2M1.

==> backup/01-introduction.tex <==
\begin{figure}[b]
    \centering
    \hfill 
    \begin{subfigure}[b]{0.7\textwidth} 
        \includegraphics[width=1.\linewidth]{figs/F9-fp4-int4-format-codebooks.pdf}
        \caption{
        Signed representable values of representative 4-bit formats.
        }
        \label{fig:fp4-int4-format-codebooks}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.28\textwidth} 
        \includegraphics[width=\textwidth]{figs/F1-longrun-relative-lm-loss-error-124B.pdf}
        \caption{Estimated EL at $1e22$ FLOPs}
        \label{fig:lever-1e22}
    \end{subfigure}
    \hfill 
    \caption{Red spans mark RTNE bins, \(\ell\) and \(r\) denote the left and right half-widths of each bin.
        Bars show the expected rounding error, with a toward-zero bias in E2M1 format but not in E1M2/INT4 format. 
    }
    \label{fig:hotmap-lever}
\end{figure}


\section{Introduction}
\label{sec:intro}

% Scaling Law 的提出与应用，使得小规模模型上的架构、数据和训练策略创新能够更可靠地外推到大规模训练，从而推动了大语言模型能力上界的持续提升。然而，完整训练一个前沿模型的成本依然极高，显存、带宽和矩阵计算吞吐已经成为继续 scaling 的关键瓶颈。因此，如何降低训练过程中的资源和显存需求，已经成为推动 LLM 继续扩展的重要问题。
% 低精度训练是降低训练成本的一条重要路径。其基本思想是在前向传播和反向传播过程中使用低精度 activation、weight 和 gradient，并借助现代硬件高效的低精度矩阵计算能力提升端到端训练吞吐。近年来，FP8 已经在多个大规模训练系统中被采用 \citep{dpsk,ling}，表明进一步降低训练精度具有现实可行性。随着硬件发展，Blackwell 等新一代加速器开始提供原生 FP4 矩阵计算路径，为进一步降低 LLM 训练成本提供了新的机会。
% 当前主流 FP4 训练接口大多围绕 E2M1 format 设计。例如，MXFP4 / NVFP4 类格式会为细粒度 tensor block 维护独立 scale，并通过不同 block size 和 scale hierarchy 在动态范围、精度和硬件效率之间折中。NVFP4 由于更小的 block 和更精细的 scale 设计，通常比 MXFP4 具有更好的训练精度。即便如此，FP4 只有 16 个可表示值，直接用于训练仍会面临严重的收敛和稳定性问题。为缓解这些问题，NVFP4 recipe 引入 Random Hadamard Transform（RHT）和 stochastic rounding 来处理 outlier 与梯度更新不稳定；后续工作则进一步从 scale 设计、rounding / gradient estimation、outlier control 和量化感知训练等方向缩小 FP4 与 BF16 之间的差距。
% 尽管现有方法显著改善了 E2M1-based FP4 training，它们大多仍默认保留 E2M1 data-element grid。本文重新审视这一默认选择。我们的核心发现是：RHT 不仅缓解 outlier，也改变了量化问题本身。RHT 将 tensor 从 dynamic-range-limited regime 推向 local-resolution-limited regime；在这一 regime 下，E2M1 的非均匀 RTNE bin 会产生 Shrinkage Bias，使 RHT 带来的 bucket utilization 提升在关键 tensor 上难以转化为更低的量化误差。相比之下，E1M2/INT4-style uniform grid 能够更好地利用 post-RHT 分布，从而获得更高的量化质量。
% 基于这一发现，我们提出 UFP4，一种面向训练的 uniform 4-bit recipe。UFP4 使用 E1M2/INT4-style uniform grid，在 fwd_y、bwd_dx 和 bwd_dw 三个 training GEMM 上全部启用 RHT，并仅在 dY 上使用 stochastic rounding。UFP4 表明，full-RHT training 本身并非问题；问题在于 E2M1 grid 与 post-RHT tensor regime 的不匹配。在 uniform grid 下，RHT 可以扩展到 forward、data-gradient 和 weight-gradient 路径，并在长跑训练中保持稳定收益。

Scaling laws have made it increasingly reliable to extrapolate architectural, data, and training-strategy improvements from small-scale experiments to large-scale language-model training.
This has accelerated iteration across the Large Language Model (LLM) stack and has repeatedly pushed the frontier of model capabilities.
Yet training a frontier model remains extremely expensive.
Memory capacity, memory bandwidth, and matrix-computation throughput are now central bottlenecks for continued scaling.
Reducing the resource and memory footprint of training is therefore a key requirement for further expanding large language models.

Low-precision training is one of the most promising approaches to this problem.
The basic idea is to represent activations, weights, and gradients in lower precision during forward and backward computation, and to leverage the low-precision matrix-multiply units in modern accelerators for high-throughput training.
FP8 has already been adopted in multiple large language models~\citep{Team2025EveryAB,DeepSeekAI2024DeepSeekV3TR}, showing that further reducing training precision can be practically viable.
With newer accelerators such as NVIDIA Blackwell exposing native FP4 matrix-computation paths, 4-bit training offers an opportunity to further reduce the cost of LLM pretraining.

Current FP4 training interfaces are largely designed around the E2M1 format.
For example, MXFP4- and NVFP4-style formats maintain independent scale information for fine-grained tensor blocks, trading off dynamic range, precision, and hardware efficiency through different block sizes and scale hierarchies.
Compared with MXFP4, NVFP4 typically provides better training accuracy through smaller blocks and a more refined scaling design.
Nevertheless, using only 16 representable values makes end-to-end FP4 training difficult: without additional stabilization, FP4 recipes can suffer from severe convergence issues and BF16-relative loss degradation.
To mitigate these problems, the NVFP4 recipe~\citep{nvidia2026pretraininglargelanguagemodels} introduces the Random Hadamard Transform (RHT) and stochastic rounding (SR) to handle outliers and stabilize gradient updates.
Recent work further reduces the gap between FP4 and BF16 training through improved scale design, rounding or gradient-estimation methods, outlier control, and quantization-aware training strategies~\citep{chen2026tetrajetv2accuratenvfp4training,panferov2026quartetiiaccuratellm,cao2025metis}.

Despite these improvements, most existing methods still keep the E2M1 data-element format unchanged.
This paper revisits that default choice.
Our central observation is that the Random Hadamard Transform (RHT) does not merely suppress outliers; it changes the quantization regime itself.
By dispersing outlier energy, RHT moves tensors from a dynamic-range-limited regime toward a local-resolution-limited regime.
In this post-RHT regime, the non-uniform rounding bins of E2M1 can introduce \emph{Shrinkage Bias}, preventing the improved bucket utilization brought by RHT from consistently translating into lower quantization error on tensors.
In contrast, an E1M2/INT4-style uniform grid better matches the post-RHT distribution and can convert the same bucket-utilization improvement into higher quantization quality.

Based on this finding, we propose \heroname{}, a uniform 4-bit training recipe built on an E1M2/INT4-style uniform grid.
\heroname{} applies RHT to the operands of all three linear-layer training GEMMs, the forward pass (FPROP, \fwdy{}), the data-gradient pass (DGRAD, \bwddx{}), and the weight-gradient pass (WGRAD, \bwddw{}), and uses stochastic rounding only when quantizing the upstream gradient \(dY\).
The recipe shows that full-RHT training is not inherently harmful; rather, the issue is the mismatch between the E2M1 grid and the post-RHT tensor regime.
With a uniform grid, RHT can be extended to forward, data-gradient, and weight-gradient paths while preserving stable long-run training gains.

We summarize our contributions as follows:
\begin{itemize}
    \item We identify a post-RHT regime shift in FP4 training and formalize \emph{Shrinkage Bias}: asymmetric E2M1 rounding bins can induce grid-level magnitude attenuation, which can propagate to GEMM-level attenuation of the coherent signal component.

    \item We show through real-tensor and single-GEMM diagnostics that RHT changes the preferred FP4 grid. E2M1 can benefit from its wider range before rotation, but after RHT, E1M2/INT4-style uniform grids more reliably convert improved bucket utilization into higher SQNR.

    \item We propose \heroname{}, a uniform-FP4 recipe that enables RHT on all three training GEMMs while keeping stochastic rounding only on \(dY\).

    \item We validate \heroname{} on Dense 1.5B, MoE 7.9B, and MoE 124B long-run pretraining, and support its robustness and practicality with scaling-law, ablation, and fused-kernel evidence, motivating uniform 4-bit grids as first-class FP4 training formats.
\end{itemize}

\clearpage

==> backup/02-background.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
% 中文意图：本章只建立记号和背景，不提前下结论。需要让读者理解 E2M1/E1M2/INT4、blockwise quantization、RHT 以及训练中三个 GEMM 的形式。避免在这里写 “E2M1 错了” 或 “UFP4 最优”。

\subsection{4-bit Formats and Blockwise Quantization}
\label{sec:prelim-quant}
% 中文意图：介绍 E2M1、E1M2、INT4 的 codebook 差异，并定义统一的 blockwise quantizer。核心是把后文所有 format comparison 固定到同一 scale convention 下。

Each 4-bit format encodes a value using one sign bit and three payload bits, which are partitioned into $x$ exponent bits and $y$ mantissa bits; we denote such formats as E$x$M$y$.
Different partitions yield different \emph{normalized codebooks}; we consider E2M1, E1M2, and INT4 (\Cref{fig:fp4-int4-format-codebooks}).

In practice, blockwise quantization is widely adopted to improve precision by partitioning a tensor \(\mathbf T\) into contiguous blocks \(\{B\}\) and mapping each element to a codebook level under a shared per-block scale.
Let \(G=\{g\}\) denote the normalized codebook of a chosen format, \(g_{\max}=\max_{g\in G}|g|\) its largest magnitude level, and \(\rho_G\) the rounding rule.  The quantization process is then:
\[
    s_B=\frac{\max_{x_j\in B}|x_j|}{g_{\max}},
    \qquad
    q_i=\rho_G\!\left(\frac{x_i}{s_B}\right)\in G.
\]
We write \(Q_G(\mathbf T)\) for the quantized tensor; in arithmetic expressions it denotes the dequantized numerical tensor.\footnote{%
  MXFP4 uses \(1{\times}32\) blocks with an E8M0 scale; NVFP4 uses \(1{\times}16\) blocks with two-level scaling.}

The rounding rule \(\rho_G\) is either Round-To-Nearest-Even (RTNE) or Stochastic Rounding (SR).
RTNE selects the nearest level in \(G\) with deterministic tie-breaking.
When \(x_i/s_B\) falls between adjacent levels \(g_a<g_b\), SR samples:
\[
    \Pr[q_i=g_b]=\frac{x_i/s_B - g_a}{g_b-g_a},
    \qquad
    \Pr[q_i=g_a]=\frac{g_b - x_i/s_B}{g_b-g_a}.
\]
SR preserves the normalized value in expectation, while RTNE is deterministic.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/F9-fp4-int4-format-codebooks.pdf}
    \caption{
    Normalized codebooks for representative 4-bit formats.
    E2M1 provides wider dynamic range with non-uniform spacing; E1M2 and INT4 distribute levels uniformly, offering finer local resolution.
    }
    \label{fig:fp4-int4-format-codebooks}
\end{figure}

\subsection{Random Hadamard transforms}
\label{sec:prelim-rht}
% 中文意图：介绍 RHT 是 norm-preserving 的 rotation，能把 outlier energy 分散到更多坐标中。随后给出 fwd_y、bwd_dx、bwd_dw 三个 GEMM 加 RHT 后的公式，为 Shrinkage Bias 和 UFP4 recipe 做铺垫。

Hadamard transforms are structured rotations applied before quantization to disperse outlier coordinates.
We use the Sylvester Hadamard matrices
\[
    \mathbf H_{1}=[1],
    \qquad
    \mathbf H_{2}=\frac{1}{\sqrt{2}}
    \begin{bmatrix}
        1 & 1\\
        1 & -1
    \end{bmatrix},
    \qquad
    \mathbf H_{2n}=\frac{1}{\sqrt{2}}
    \begin{bmatrix}
        \mathbf H_n & \mathbf H_n\\
        \mathbf H_n & -\mathbf H_n
    \end{bmatrix},
\]
so \(\mathbf H_n^\top\mathbf H_n=I_n\) for \(n=2^k\).
An RHT additionally applies a fixed random sign matrix before the Hadamard transform:
\[
    \mathbf H'_n=\mathbf S_n\mathbf H_n,
    \qquad
    \mathbf S_n=\operatorname{diag}(\epsilon_1,\ldots,\epsilon_n),
    \qquad
    \epsilon_i\in\{-1,+1\}.
\]
Since \(\mathbf H'_n\) is orthogonal, applying the same transform to the shared GEMM dimension preserves the full-precision result:
\[
    \mathbf Y=\mathbf X\mathbf W^\top
    =
    (\mathbf X\mathbf H'_n){(\mathbf W\mathbf H'_n)}^{\top}.
\]
The corresponding low-precision RHT GEMM quantizes the rotated operands,
\[
    \widehat{\mathbf Y}
    =
    Q_G(\mathbf X\mathbf H'_n)\,
    {Q_G(\mathbf W\mathbf H'_n)}^{\top},
\]
where \(Q_G(\cdot)\) denotes the dequantized numerical tensor associated with the blockwise representation in \Cref{eq:block-quantizer}.
RHT reduces outlier dominance before quantization, but its effect on quantization error depends on the FP4 grid.
For the three training GEMMs, RHT is applied along the shared reduction dimension: the input-channel dimension for \fwdy{}, the output-channel dimension for \bwddx{}, and the batch-token dimension for \bwddw{}.


==> backup/03-mechanism.tex <==

% ======================================================================
\section{Shrinkage Bias in 4-bit Format Grids}
\label{sec:shrinkage-bias}
% 中文意图：本章是全文机制核心。目标是用保守数学推导说明 E2M1 非均匀 grid 在 normalized magnitude space 中会产生负的期望量化误差，并讨论该偏差如何进入 GEMM 主信号。不要写成 universal theorem，也不要把 tensor norm contraction 当作 Shrinkage Bias 的定义。

\subsection{Shrinkage Bias from asymmetric RTNE bins}
\label{sec:cell-contraction}
% 中文意图：用 rounding-bin asymmetry 形式化 E2M1 的 Shrinkage Bias。重点不是“任意分布都会 shrink”，而是 E2M1 的某些 codepoint 不在自己的 RTNE bin 中心；因此即使 bin 内局部分布均匀，也会产生非零期望幅值误差。E1M2/INT4 的均匀 interior bins 消除了这个 grid-geometry source。该节只讨论固定 scale、无 clipping 的 RTNE 机制；SR、clipping、scale estimation 作为额外因素留给实验和讨论。

Fix a block scale \(s\), and write \(t=|x|/s\) for values within the representable range.
We analyze the positive normalized magnitudes; the corresponding unnormalized error is multiplied by \(s\).
For brevity, \(Q(t)\) denotes RTNE rounding to the nearest normalized quantization level.
Let the positive normalized magnitudes of a format be
\[
    0 = q_0 < q_1 < \cdots < q_n .
\]
For an interior quantization level \(q_i\), the interior of its RTNE rounding bin is
\begin{equation}
    \mathcal{B}_i
    =
    \left(
    \frac{q_{i-1}+q_i}{2},
    \frac{q_i+q_{i+1}}{2}
    \right),
    \qquad
    \ell_i=\frac{q_i-q_{i-1}}{2},
    \quad
    r_i=\frac{q_{i+1}-q_i}{2},
    \label{eq:rtn-bin}
\end{equation}
where \(\ell_i\) and \(r_i\) are the left and right bin widths around \(q_i\).
For a positive magnitude \(t\in\mathcal{B}_i\), the magnitude error is \(Q(t)-t=q_i-t\).
If the density inside this bin is locally uniform, the conditional expected error is
\begin{equation}
    \mathbb{E}\!\left[Q(t)-t \mid t\in\mathcal{B}_i\right]
    =
    \frac{1}{\ell_i+r_i}
    \int_{-\ell_i}^{r_i} (-u)\,du
    =
    \frac{\ell_i-r_i}{2}
    =
    \frac{2q_i-q_{i-1}-q_{i+1}}{4}.
    \label{eq:bin-asymmetry-bias}
\end{equation}
Thus, a quantization level whose RTNE bin is wider on the right than on the left has a negative expected magnitude error even under locally uniform bin occupancy.
This is a grid-geometry source of magnitude shrinkage, distinct from distribution-induced quantization error inside a symmetric bin.

E2M1 contains such asymmetric bins at spacing-transition points.
For example, with positive magnitudes \(\{0, 0.5, 1, 1.5, 2, 3, 4, 6\}\), the quantization level \(q=2\) has bin \((1.75,2.5)\), so \(\ell=0.25\) and \(r=0.5\).  Equation~\eqref{eq:bin-asymmetry-bias} gives
\[
    \mathbb{E}[Q(t)-t \mid t\in(1.75,2.5)]
    =
    -0.125 .
\]
The \(q=4\) bin has the same shrinkage-inducing asymmetry with a larger scale.
By contrast, the E1M2/INT4 grids are uniformly spaced and satisfy
\[
    q_{i+1}-q_i = q_i-q_{i-1}
\]
for interior bins, hence \(\ell_i=r_i\) and the asymmetry term in Equation~\eqref{eq:bin-asymmetry-bias} is zero.

This does not mean that E1M2/INT4 is unbiased for every possible distribution:
a skewed density within a bin can still create distribution-induced error.
Motivated by the bin-level expectation above, we define \emph{Shrinkage Bias} as negative expected RTNE error in normalized magnitude space: for a distribution \(\mathcal{P}\) over \(t=|x|/s\), let \(b_G(\mathcal{P})=\mathbb{E}_{t\sim\mathcal{P}}[Q(t)-t]\), and \(b_G(\mathcal{P})<0\) indicates Shrinkage Bias.
Under this definition, E2M1 introduces a format-level source of \emph{Shrinkage Bias} whenever tensor mass occupies asymmetric bins, while uniform 4-bit grids remove this bin-asymmetry source under the same scale convention.

\subsection{Propagation through Matrix Multiplication}
\label{sec:gemm-bias-propagation}
% 中文意图：用严格的 projection decomposition 表达 operand-level attenuation 如何进入 GEMM 主信号。单次 GEMM 部分是恒等式；多次 GEMM 部分只作为 residual-incoherence 假设下的 propagation model，不写成无条件训练收敛定理。

The bin-level bias above becomes relevant to training only if it survives tensor aggregation and enters linear-layer computations.
For a General Matrix Multiplication (GEMM) \(Z=AB^\top\), let the dequantized low-precision operands be \(\widehat{A}=Q_G(A)\) and \(\widehat{B}=Q_G(B)\).
We measure operand-level attenuation by projecting each quantized operand onto its BF16 counterpart:
\begin{equation}
    \alpha_A
    =
    \frac{\langle \widehat{A},A\rangle_F}{\|A\|_F^2},
    \qquad
    \widehat{A}
    =
    \alpha_A A + R_A,
    \qquad
    \langle R_A,A\rangle_F=0,
    \label{eq:operand-projection-a}
\end{equation}
and analogously \(\widehat{B}=\alpha_B B+R_B\) with \(\langle R_B,B\rangle_F=0\).
When \(\alpha_A<1\), the quantized operand has a smaller component aligned with \(A\); this is the tensor-level counterpart of magnitude shrinkage.

Substituting the decompositions into the quantized GEMM gives the exact identity
\begin{equation}
    Z_q
    =
    \widehat{A}\widehat{B}^{\top}
    =
    \alpha_A\alpha_B AB^\top
    +
    \alpha_A A R_B^\top
    +
    \alpha_B R_A B^\top
    +
    R_A R_B^\top .
    \label{eq:gemm-propagation}
\end{equation}
The first term contains a coherent copy of the BF16 GEMM output \(Z\).
If the residual terms are relatively incoherent with \(Z\), the dominant signal is attenuated by approximately
\[
    Z_q \approx \alpha_A\alpha_B Z + \text{residual noise}.
\]

The same projection diagnostic can be applied along non-leaf paths.
Suppose a local linearized path contains \(K\) quantized GEMMs.
For the \(k\)-th GEMM, let \(\eta_k\) denote its coherent attenuation factor, i.e., the projection of the quantized GEMM output onto the corresponding clean output.  For a single GEMM, \(\eta_k\) is approximately \(\alpha_{A,k}\alpha_{B,k}\), up to any residual projection onto the clean output.
Under the same residual-incoherence approximation, the clean signal component after the path is scaled by
\begin{equation}
    \prod_{k=1}^{K}\eta_k
    =
    \prod_{k=1}^{K}(1-\delta_k)
    \approx
    \exp\!\left(-\sum_{k=1}^{K}\delta_k\right),
    \qquad
    \delta_k=1-\eta_k .
    \label{eq:multi-gemm-attenuation}
\end{equation}
The exponential form uses \(\log(1-\delta_k)=-\delta_k+O(\delta_k^2)\) for \(|\delta_k|\ll1\); when \(0<\eta_k<1\), \(\delta_k\) is the per-GEMM coherent signal loss.
Thus, a small systematic shrinkage can accumulate multiplicatively rather than cancel like zero-mean noise.
We use this as a DAG-aware projection diagnostic and propagation hypothesis, not as a standalone convergence theorem.
Quantization errors in the \fwdy{} and \bwddx{} GEMM outputs are non-leaf errors consumed by later layers in the same step, whereas errors in \bwddw{} are leaf-gradient errors consumed by the optimizer.

\subsection{Shrinkage Bias after RHT}
\label{sec:shrinkage-after-rht}
% 中文意图：解释 RHT 后为什么问题暴露。pre-RHT 下 E2M1 dynamic range 合理；post-RHT 后 tensor 变 concentrated，local resolution 主导，E2M1 的宽 cell 变成问题。加入 shrinkage-region mass 和 bucket entropy 两个指标，服务后续真实 tensor 分析。

Before rotation, E2M1 is a sensible choice for outlier-heavy tensors: its wider dynamic range can reduce saturation.
RHT changes the regime.  Because RHT spreads outlier energy across coordinates while preserving norm, the transformed tensor is less dynamic-range-limited and more local-resolution-limited.
In this post-RHT regime, the question is no longer only whether the format can represent extreme outliers; it is whether it preserves the dense mass near the typical magnitude.

We formalize the real-tensor analysis using two metrics.
First, we measure utilization over quantized magnitude levels, which we call buckets for this metric and include the zero bucket.
Let \(K\) be the number of magnitude buckets and let \(p_i\) be the empirical fraction of quantized entries assigned to bucket \(i\).
The unnormalized bucket entropy and normalized bucket entropy are
\begin{equation}
    \mathcal{E}(G,T)
    =
    -\sum_{i=1}^{K} p_i \log(p_i+\epsilon),
    \qquad
    U(G,T)
    =
    \frac{\mathcal{E}(G,T)}{\log K}.
    \label{eq:bucket-entropy}
\end{equation}
In the experiments below we report the entropy-derived effective bucket ratio
\begin{equation}
    B_{\mathrm{eff}}(G,T)
    =
    \frac{\exp(\mathcal{E}(G,T))}{K}
    =
    K^{U(G,T)-1}.
    \label{eq:effective-bucket-ratio}
\end{equation}
\(B_{\mathrm{eff}}=1\) when all magnitude buckets are used uniformly, and \(B_{\mathrm{eff}}=1/K\) when all values collapse into a single bucket.

To compare quantization quality across tensors with different raw error scales, we report normalized mean squared error.
Let \(A\in\{I,\mathbf{H}_{16}\}\), where \(I\) denotes the identity matrix and \(\mathbf{H}_{16}\) denotes the Hadamard matrix with block size 16.
We define
\begin{equation}
    \mathrm{NMSE}_{A}(G,T)
    =
    \frac{\|Q_G(TA)-TA\|_F^2}{\|TA\|_F^2},
    \qquad A\in\{I,\mathbf{H}_{16}\}.
    \label{eq:nmse}
\end{equation}
Thus, \(\mathrm{NMSE}_{I}\) is the raw-domain quantization error, and \(\mathrm{NMSE}_{\mathbf{H}_{16}}\) is the post-RHT quantization error.
We then summarize the RHT-induced change using
\begin{equation}
    \Delta\mathrm{SQNR}
    =
    10\log_{10}
    \frac{\mathrm{NMSE}_{I}}{\mathrm{NMSE}_{\mathbf{H}_{16}}},
    \label{eq:delta-sqnr}
\end{equation}
where positive values indicate that RHT improves tensor-level signal-to-quantization-noise ratio.

% 图 4 展示了我们基于真实数据针对 MLP linear_fc1 (gate_proj, up_proj) 和 linear_fc2 (down_proj) 相关 tensor 的分析，包括 fwd_w (weight)、fwd_x (input) 和 bwd_dy (output gradient)。
% 数据显示，RHT 对于 linear_fc1/bwd_dy 和 linear_fc2/fwd_x 这两类高坍缩张量能有效提高 effective bucket ratio，这与 Swiglu 存在放大 outlier 的现象一致。
% 但相反的是，E2M1 精度下 RHT 会显著降低 \(\Delta\mathrm{SQNR}\)，而 E1M2 精度下 \(\Delta\mathrm{SQNR}\) 往往是正的。
% 这说明 RHT 作用于 E2M1 非均匀网格会引入更多量化噪声，而作用于 E1M2 均匀网格则能把更好的 bucket 利用率转换为更好的量化质量。
% 这些现象也印证了为什么社区诸多基于 E2M1 的训练方法提到 RHT 应用于 fwd_y, bwd_dx 计算过程对训练效果有损。

\Cref{fig:rht-bucket-sqnr-tradeoff} analyzes real training tensors from MLP \texttt{linear\_fc1} (\texttt{gate\_proj}, \texttt{up\_proj}) and \texttt{linear\_fc2} (\texttt{down\_proj}), covering \texttt{fwd\_w}, \texttt{fwd\_x}, and \texttt{bwd\_dy}. 
RHT substantially increases the effective bucket ratio for outlier-heavy tensors, particularly \texttt{linear\_fc1}/\texttt{bwd\_dy} and \texttt{linear\_fc2}/\texttt{fwd\_x}, consistent with the outlier-amplifying behavior of SwiGLU activation \citep{Jiang2026PowLUAA}.
However, this improved bucket utilization has opposite effects under the two 4-bit grids: with E2M1, RHT often decreases \(\Delta\mathrm{SQNR}\), while with E1M2, \(\Delta\mathrm{SQNR}\) is typically positive.

This indicates that RHT alone is not sufficient; its effect depends on the grid to which the rotated tensor is quantized. 
Under the non-uniform E2M1 grid, post-RHT concentrated tensors incur additional quantization noise, whereas the uniformly spaced E1M2 grid converts the improved bucket utilization into higher quantization quality. 
This tensor-level evidence helps explain why applying RHT to non-leaf paths such as \texttt{fwd\_y} and \texttt{bwd\_dx} can hurt E2M1-based training recipes, despite RHT being effective at outlier dispersion.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/F31-rht-utilization-sqnr-tradeoff-grid-layercolor-step30000_layers1_23_fc1_fc2.pdf}
    \caption{
    RHT-induced changes in effective bucket ratio and SQNR on real training tensors, 
    where colors distinguish E2M1 and E1M2, while opacity increases with layer depth.
    \texttt{fwd\_w}, \texttt{fwd\_x}, and \texttt{bwd\_dy} denote the weight, input, and output-gradient tensors of linear layers, respectively.
    }
    \label{fig:rht-bucket-sqnr-tradeoff}
\end{figure}


% \subsection{Community remedies and their scope}
% \label{sec:community-remedies}
% 中文意图：这里不写长 Related Work，只用 1 段把社区方法按层级分类。重点是说明很多工作缓解的是 rounding、scale、tensor distribution，但保留 E2M1 grid，因此不能从根上消除本文定义的 grid-induced Shrinkage Bias。所有具体论文引用后续由 Related Work 补。

% Existing FP4 training methods can be viewed as attempts to mitigate the same failure mode at different levels.  Quantizer-side methods modify rounding rules, scale updates, or backward alignment to reduce deterministic error or variance.  Tensor-side methods decompose, smooth, or separate difficult components before quantization.  These techniques can be valuable and are largely orthogonal to \heroname{}.  However, if the final data-element grid remains E2M1, the residual tensor is still mapped onto a non-uniform grid whose geometry can produce post-RHT contraction.  \heroname{} therefore takes the complementary route: it changes the data-element grid itself.

% ======================================================================
\section{\heroname{}: Uniform 4-bit Linear Layers with Unbiased Gradients}
\label{sec:ufp4}

% 当下广泛被采用的 FP4 Recipe 大都基于 E2M1 的数据格式，受限于 IEEE 754 标准及软硬件约束，社区中诸多缓解 FP4 训练误差的方法均无法从根源上消除 Shrinkage Bias。
% UFP4 是一种建立在 E1M2/INT4 数据格式基础上的 4-bit 训练 Recipe，其核心思路如图所示：
% 1. 对于 fwd_x, fwd_w, bwd_dy 等 tensor 在 GEMM 计算前均执行 RHT 变换并量化到 INT4 精度中
% 2. 此外，SR 应用于 bwd_dy 来保障梯度更新方向的无偏性
% UFP4 Recipe 在 RHT + 等间距 E1M2/INT4 格式下提供了一种新的 4bit 训练 Recipe 的视角，它足够的简单、高效且具备更优的训练精度。我们倡导各家厂商重新重视 E1M2/INT4，并在未来的高性能训练卡上完成支持。
% 针对 scale 精度选择与本文关注的目标是正交的（例如 scale 使用一级量化（mxfp4 1*16 E8M0 scale）或者二级量化（nvfp4 1*16 E4M3 scale + global FP32 scale）或者三级量化（HiFloat4）），scale 的设计应该在精度可靠范围内选择最贴合硬件计算效率的方案。

Most existing FP4 training recipes are built around the E2M1 data format \citep{nvidia2026pretraininglargelanguagemodels,chen2026tetrajetv2accuratenvfp4training,panferov2026quartetiiaccuratellm}. 
While this choice is attractive for raw outlier-heavy tensors, many existing mitigation techniques only modify rounding, scaling, rotation placement, or tensor preprocessing, leaving the E2M1 grid geometry unchanged. 
They can therefore reduce the symptoms of \emph{Shrinkage Bias}, but they do not remove its format-level source.

The diagnosis above suggests a simple design principle: after RHT has moved tensors from a dynamic-range-limited regime to a local-resolution-limited regime, the 4-bit quantization grid should prioritize local magnitude preservation over extra dynamic range.
Therefore, we propose \heroname{}, a uniform 4-bit training recipe based on an E1M2/INT4-style uniform grid, as shown in Figure~\ref{fig:ufp4-recipe-overview}.
For each linear-layer GEMM, \heroname{} applies RHT to the relevant operands and quantizes them to a uniformly spaced 4-bit grid. 
Unlike E2M1 recipes that typically restrict RHT to the weight-gradient path, \heroname{} enables RHT for all three GEMMs: FPROP(\fwdy{}), DGRAD(\bwddx{}), and WGRAD(\bwddw{}).
Stochastic rounding is applied to \(dY\) to preserve the gradient direction in expectation.

The scale hierarchy is orthogonal to this format-level argument: one may use single-level, two-level, or hierarchical scales depending on hardware efficiency, as long as accuracy is preserved. 
Our main recommendation is that future training accelerators should support E1M2/INT4-style uniform 4-bit grids as first-class training data elements, rather than treating E2M1 as the only serious FP4 training choice.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/ufp4-recipe-overview.png}
    \caption{
    Overview of the \heroname{} recipe.
    }
    \label{fig:ufp4-recipe-overview}
\end{figure}

